Galactic transient sources with the Cherenkov Telescope Array Observatory

A wide variety of Galactic sources show transient emission at soft and hard X-ray energies: low- and high-mass X-ray binaries containing compact objects, isolated neutron stars exhibiting extreme variability as magnetars as well as pulsar-wind nebulae. Although most of them can show emission up to MeV and/or GeV energies, many have not yet been detected in the TeV domain by Imaging Atmospheric Cherenkov Telescopes. In this paper, we explore the feasibility of detecting new Galactic transients with the Cherenkov Telescope Array Observatory (CTAO) and the prospects for studying them with Target of Opportunity observations. We show that CTAO will likely detect new sources in the TeV regime, such as the massive microquasars in the Cygnus region, low-mass X-ray binaries with low-viewing angle, flaring emission from the Crab pulsar-wind nebula or other novae explosions, among others. Since some of these sources could also exhibit emission at larger time-scales, we additionally test their detectability at longer exposures. We finally discuss the multiwavelength synergies with other instruments and large astronomical facilities.

==> synergies_old.tex <==
\section{Synergies with large astronomical facilities} \label{sec:synergies}
%\textbf{Maybe shorten the section a little bit...}
%%%%%%
%ALO 
Simultaneous coordinated observations with telescopes and facilities at different wavelengths are crucial for understanding the processes and mechanisms at work in the sources of our interest (see \citealp{2019sCTA.book.....C} for a detailed review). Coordination, response to real-time alerts and target-of-opportunity (ToOs) are key in time domain astrophysics when observing transient events. In the case of Galactic transients, external alerts can trigger ToO observations by CTAO of new Galactic events or renewed activity of known sources. The trigger criteria is dependent on the type of source observed, with different time urgency and duration varying in terms of the evolution of the specific phenomena. {We recommend CTAO to participate in} 
%The participation of CTAO in 
networks (such as  the Astrophysical Multi-messenger Observatory Network, AMON\footnote{\url{https://www.amon.psu.edu/}} or Simultaneous Multiwavelenth Astronomy Research in Transients NETwork, SMARTNet \citealp{2017NewAR..79...26M})
%, would 
to increase the chances of coordination and follow-up in a multi-wavelength and multi-messenger context. 

The radio band is of general interest for providing information of the non-thermal processes, and radio facilities are key for locating acceleration sites and shocks. %such as ALMA or EHT are key for locating acceleration sites and shocks. 
Among other discoveries, the recent association of a \textbf{Galactic} magnetar and a FRB has proven that magnetars are the engines of at least some FRBs. FRB-like events triggered in radio will be key to search for (short-timescale) VHE counterparts of, at least, some magnetar engines. For that purpose, {CTAO} will need an external trigger from a radio observatory sensitive to millisecond bursts and capable of issuing prompt alerts. Current generation of telescopes like CHIME, with a large field of view and collecting area, have proven to be excellent detectors for FRB events. Similarly, MeerKat (and future SKA), with its MeerTRAP project to continuously search and detect this type of millisecond-duration events, will provide the needed trigger. Other facilities such ALMA will share important synergies with CTAO.

In the optical and infrared domain prompt reaction would be facilitated by coordinating with external observatories within time zones close to those of CTAO sites. In the case of CTAO North, {it} should be pursuing synergies mainly with La Palma, Tenerife (and CAHA) telescopes in Spain, while in the CTAO South the most appropriate choice would be the different ESO telescopes and other large facilities in Chile, such as the Rubin Observatory Legacy Survey of Space and Time (LSST), which will be key for time-domain astronomy \citep[see][]{2022arXiv220804499H}. 
%The telescope array BlackGEM \footnote{\url{https://astro.ru.nl/blackgem/}} and the he Gravitational-wave Optical Transient Observer (GOTO)\footnote{\url{https://goto-observatory.org/}} will perform optical counterpart identification of gravitational wave events, providing wide field transient discovery in the GW era. 
The availability of imaging and spectroscopic instrumentation in both hemispheres {does} largely fulfill the observational needs required for coordinated campaigns. Specific target of opportunity proposals could be eventually placed by the CTAO community. In parallel, small optical telescopes either on-site or operated by nearby CTAO institutions could also play a key role in this effort if the targets are bright enough as in the case of novae or gamma-ray binaries. This could serve to mitigate the often high time pressure on large telescopes. Additionally, support optical telescopes would ensure a fast follow-up on transients and would provide sufficient coverage in the case of bright sources.

%Future s
Space missions will allow to study the X-ray domain with improved capabilities. The Space Variable Objects Monitor (SVOM) %is expected to be launched in mid {2024} 
has been recently launcghed to study GRBs in the 4 - 150 keV range. Although its science is focused in GRB detection, it is likely that it will also detect outbursts or GRB-like events of Galactic origin, i.e., magnetar giant flares. The Advanced Telescope for High-ENergy Astrophysics (Athena) is scheduled for launch in {mid} 2030s. It will operate in the energy range of 0.2–12 keV. This and other future observatories will be key in Galactic transient detection. As an example, it was seen that changes in the hardness of the X-ray emission of magnetars could be an indicator of an incoming FRB-like event {\citep{2020ApJ...898L..29M}}, which might allow to trigger observations by CTAO if confirmed. 

The high-energy band (E$>$100 MeV) is currently explored by the \textit{Fermi}-LAT satellite. Triggers from \textit{Fermi}-LAT have been important for the detection of AGNs and novae in the VHE domain, among others. MeV-GeV information provided with simultaneous observations with Fermi is also important to disentangle between hadronic and leptonic processes. If \textit{Fermi} lifetime extends through (at least partially) CTAO lifetime, it will provide the needed coverage and alerts to certain observations/triggers. {Just recently, the AGILE satellite, that also operated in this energy range, ceased its operations and re-entered the atmosphere \citep{AGILE2024}.}  For the moment, there is no obvious successor to Fermi {or AGILE} in the same energy domain, although some missions could take over. {A successor will be crucial to fully exploit the full potential of gamma-ray astronomy.} The High Energy cosmic-Radiation Detection facility (HERD) is expected to be operational from 2026 on board of the Chinese Space Station, detecting gamma rays above 0.5 GeV.

Finally, in a multi-messenger context, CTAO will be able to search for the electromagnetic counterpart of GWs generated in the Milky Way, such as white dwarf binary mergers. The Laser Interferometer Space Antenna (LISA) mission will be the first GW observatory on space (scheduled launch on 2030) and will key to study white dwarf mergers \citep{2019MNRAS.490.5888L,2023MNRAS.519.2552G}. CTAO could potentially follow-up transient alerts to search for a putative counterpart. {Finally, neutrino alerts will also be crucial in the case some events such as e.g. Galactic core-collapse supernovae.}

\textbf{Regarding the observational strategy, a first description on the triggering criteria, expected trigger rate and target priority was already provided in \cite{2019sCTA.book.....C}. The specific criteria will be fully settled once the observatory is operational and will depend on the evolution of the field... WORK IN PROGRESS\\
In many cases a fast repositioning and... \\
ADD info updated table Science updates\\
Transient Handler (LST, CTAO)\\
Reference to Ulisses document?\\}


